Black is to Criminal as Caucasian is to Police: Detecting and Removing Multiclass Bias in Word Embeddings

Online texts -- across genres, registers, domains, and styles -- are riddled with human stereotypes, expressed in overt or subtle ways. Word embeddings, trained on these texts, perpetuate and amplify these stereotypes, and propagate biases to machine learning models that use word embeddings as features. In this work, we propose a method to debias word embeddings in multiclass settings such as race and religion, extending the work of (Bolukbasi et al., 2016) from the binary setting, such as binary gender. Next, we propose a novel methodology for the evaluation of multiclass debiasing. We demonstrate that our multiclass debiasing is robust and maintains the efficacy in standard NLP tasks.

==> analogy.tex <==
\begin{table}[]
    \centering
    \begin{adjustbox}{width=\linewidth}
    \begin{tabular}{c|c|c||c|c}
        Dataset & Type & Overall & Syn. & Sem. \\
        \hline
        \multirow{3}{*}{Reddit.us} & Original & 37.5 & 16.9 & 46.2 \\
        & Hard (G), $k=1$ & 37.8 & 17.9 & 46.2 \\
        & Hard (G), $k=2$ & 37.2 & 17.0 & 45.7 \\
        \hline
        \multirow{3}{*}{w2v-GoogleNews} & Original & 72.9 & 88.8 & 72.1 \\
        & Hard (G), $k=1$ & 72.7 & 86.0 & 72.0 \\
        & Hard (G), $k=2$ & 72.9 & 86.7 & 72.3 \\
    \end{tabular}
    \end{adjustbox}
    \caption{Caption}
    \label{tab:analogy_gender}
\end{table}

==> neighbor_plots.tex <==

\begin{figure*}
    \centering
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\linewidth]{cluster_images/religion-k1/jew_neighbor_plot.png}
        \caption{$k=1$}
    \end{subfigure}
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\linewidth]{cluster_images/religion-k2/jew_neighbor_plot.png}
        \caption{$k=2$}
    \end{subfigure}
    % \begin{subfigure}{\textwidth}
    %     \includegraphics[width=\linewidth]{cluster_images/religion-k3/jew_neighbor_plot.png}
    %     \caption{$k=3$}
    % \end{subfigure}
    \caption{Plots of number of neighbors to ``jew'' for each profession as a function of its original bias with respect to ``jew'', before and after debiasing, for different subspace dimensionalities.}
\end{figure*}

\begin{figure*}
    \centering
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\linewidth]{cluster_images/religion-k1/muslim_neighbor_plot.png}
        \caption{$k=1$}
    \end{subfigure}
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\linewidth]{cluster_images/religion-k2/muslim_neighbor_plot.png}
        \caption{$k=2$}
    \end{subfigure}
    % \begin{subfigure}{\textwidth}
    %     \includegraphics[width=\linewidth]{cluster_images/religion-k3/muslim_neighbor_plot.png}
    %     \caption{$k=3$}
    % \end{subfigure}
    \caption{Plots of number of neighbors to ``muslim'' for each profession as a function of its original bias with respect to ``muslim'', before and after debiasing, for different subspace dimensionalities.}
\end{figure*}

==> neighbor_tables.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|}
        \hline
        $k$ & $r$ & $\rho$ \\
        \hline
        0 & 0.767 & 0.875 \\
        1 & 0.795 & 0.891 \\
        2 & 0.718 & 0.756 \\
        3 & 0.736 & 0.772 \\
        \hline
    \end{tabular}
    \caption{Pearson's $r$ and Spearman's $\rho$ correlation coefficients between the number of biased neighbors and the original bias of professions with respect to ``jew''. All correlation coefficients have $p$-values $< 10^{-30}$.}
    \label{tab:correlation_neighbors_jew}
\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|}
        \hline
        $k$ & $r$ & $\rho$ \\
        \hline
        0 & 0.925 & 0.947 \\
        1 & 0.835 & 0.841 \\
        2 & 0.825 & 0.831 \\
        3 & 0.832 & 0.839 \\
        \hline
    \end{tabular}
    \caption{Pearson's $r$ and Spearman's $\rho$ correlation coefficients between the number of biased neighbors and the original bias of professions with respect to ``christian''. All correlation coefficients have $p$-values $< 10^{-30}$.}
    \label{tab:correlation_neighbors_christian}
\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|}
        \hline
        $k$ & $r$ & $\rho$ \\
        \hline
        0 & 0.858 & 0.894 \\
        1 & 0.774 & 0.812 \\
        2 & 0.715 & 0.721 \\
        3 & 0.712 & 0.718 \\
        \hline
    \end{tabular}
    \caption{Pearson's $r$ and Spearman's $\rho$ correlation coefficients between the number of biased neighbors and the original bias of professions with respect to ``muslim''. All correlation coefficients have $p$-values $< 10^{-30}$.}
    \label{tab:correlation_neighbors_muslim}
\end{table}

==> sentiment_analysis.tex <==
For further evaluation of our debiased embeddings on downstream tasks, we used the debiased embeddings in a binary sentiment classification task, on the Movie Review dataset \cite{pang2004}. All sequences were truncated or padded to 200 tokens in length, and classified using a single-layer LSTM with 128 hidden units. The embeddings used had 50 dimensions. As shown in Table \ref{tab:movie_review}, 

\begin{table}[]
    \centering
    \begin{tabular}{|c||c|c|}
        \hline
        Targets & $k$ & Test Acc. \\
        \hline
        Original & - & 0.53 \\
        \multirow{3}{*}{Religion (3)} & 1 & 0.5 0.54 \\
        & 2 & 0.47 0.47 \\
        & 3 & 0.5  0.55 \\
        \hline
        \multirow{3}{*}{Race (3)} & 1 & 0.54 0.57 \\
        & 2 & 0.55 0.58 \\
        & 3 &   \\
        \hline
        \multirow{3}{*}{Gender (2)} & 1 & 0.51  \\
        & 2 & 0.51 0.565 \\
        \hline
    \end{tabular}
    \caption{Test accuracy for the binary sentiment classification task on the Movie Review dataset \cite{pang2004}, using frozen original word embeddings and debiased word embeddings with respect to \textit{jew}.}
    \label{tab:movie_review}
\end{table}

==> similarity.tex <==
\begin{table}[]
    \centering
    \begin{adjustbox}{width=\linewidth}
    \begin{tabular}{c|c||c|c}
        Dataset & Type & Pearson's $r$ & Spearman's $\rho$ \\
        \hline
        \multirow{3}{*}{Reddit.us} & Original & 0.1783 & 0.1515 \\
        & Hard (G), $k=1$ & 0.1797 & 0.1525 \\
        & Hard (G), $k=2$ & 0.1762 & 0.1493 \\
        \hline
        \multirow{3}{*}{w2v-GoogleNews} & Original & 0.4558 & 0.4443 \\
        & Hard (G), $k=1$ & 0.4573 & 0.4463 \\
        & Hard (G), $k=2$ & 0.4606 & 0.4482 \\
    \end{tabular}
    \end{adjustbox}
    \caption{Caption}
    \label{tab:similarity_gender}
\end{table}
